An N2HDM Solution for the possible 96 GeV Excess

We discuss a ~3 sigma signal (local) in the light Higgs-boson search in the diphoton decay mode at ~96 GeV as reported by CMS, together with a ~2 sigma excess (local) in the bb final state at LEP in the same mass range. We review the interpretation of this possible signal as a Higgs boson in the 2~Higgs Doublet Model with an additional real Higgs singlet (N2HDM). It is shown that the lightest Higgs boson of the N2HDM can perfectly fit both excesses simultaneously, while the full Higgs-boson sector is in agreement with all Higgs-boson measurements and exclusion bounds as well as other theoretical and experimental constraints. It is demonstrated that in particular the N2HDM type~II and can fit the data best, leading to a supersymmetric interpretation. The NMSSM and the munuSSM are briefly reviewed in this respect.

==> preprint.tex <==
IFT--UAM/CSIC--19-064\\
%arXiv:1411.6526 [hep-ph]

